Parareal computation of stochastic differential equations with time-scale separation: a numerical study

The parareal algorithm is known to allow for a significant reduction in wall clock time for accurate numerical solutions by parallelising across the time dimension. We present and test a micro-macro version of parareal, in which the fine propagator is based on a (high-dimensional, slow-fast) stochastic microscopic model, and the coarse propagator is based on a low-dimensional approximate effective dynamics at slow time scales. At the microscopic level, we use an ensemble of Monte Carlo particles, whereas the approximate coarse propagator uses the (deterministic) Fokker-Planck equation for the slow degrees of freedom. The required coupling between microscopic and macroscopic representations of the system introduces several design options, specifically on how to generate a microscopic probability distribution consistent with a required macroscopic probability distribution and how to perform the coarse-level updating of the macroscopic probability distribution in a meaningful manner. We numerically study how these design options affect the efficiency of the algorithm in a number of situations. The choice of the coarse-level updating operator strongly impacts the result, with a superior performance if addition and subtraction of the quantile function (inverse cumulative distribution) is used. How microscopic states are generated has a less pronounced impact, provided a suitable prior microscopic state is used.

==> couplings.tikz.tex <==
\newif\ifincZ
\incZtrue
\newif\ifdirect
\directfalse
\begin{tikzpicture}[auto]
\tikzset{node distance=2cm}
% nodes
\node (X)   [circle]              {$\mathcal{X}$};
\node (mu)  [circle, right=of X]  {$\mu$};
\node (rho) [circle, below=of mu] {$\rho$};
\ifincZ
  \node (Z)   [circle, below=of X]  {$\mathcal{Z}$};
\fi
\node (microscopic)  [left=of X]                          {microscopic};
\node (macroscopic)  [below=of microscopic]               {macroscopic};
\node (particle)     [above=of X, rotate=90, anchor=mid]  {particle};
\node (distribution) [above=of mu, rotate=90, anchor=mid] {distribution};
% arrows
\ifdirect
  \draw [->, out=120,in=-30] (rho.north)     to node [swap] {$\oper{M}{c}{p}$} (X.east);
  \draw [-,  out=30,in=90]   (X.north east)  to ($(X)!.5!(mu)$);
  \draw [->, out=-90,in=-30] ($(X)!.5!(mu)$) to (X.east);
\else
  \draw [->, out=60,in=-60]   (rho.north east)  to node [swap] {$\oper{M}{c}{f}_1$} (mu.south east);
  \draw [-,  out=-120,in=180] (mu.south)        to ($(rho)!.5!(mu)$);
  \draw [->, out=0,in=-60]    ($(rho)!.5!(mu)$) to (mu.south east);
  \draw [->, out=150,in=30]   (mu.north west)   to node [swap] {$\oper{M}{f}{p}_2$} (X.north east);
  \draw [-,  out=-30,in=-90]  (X.east)          to ($(X)!.5!(mu)$);
  \draw [->, out=90,in=30]    ($(X)!.5!(mu)$)   to (X.north east);
  \draw [->, out=-30,in=-150] (X.south east)    to node [swap] {} (mu.south west);
\fi  

\ifincZ
  \draw [->, out=-120,in=120] (X.south west)  to node [swap] {$\oper{R}{p}{n}_1$} (Z.north west);
  \draw [->, out=-30,in=-150] (Z.south east)  to node [swap] {$\oper{R}{n}{c}_2$} (rho.south west);
\else
  \draw [->, out=-60,in=150]  (X.south)       to node [swap] {$\oper{R}{p}{c}$} (rho.west);
\fi
\end{tikzpicture}


==> for arXiv/couplings.tikz.tex <==
\newif\ifincZ
\incZtrue
\newif\ifdirect
\directfalse
\begin{tikzpicture}[auto]
\tikzset{node distance=2cm}
% nodes
\node (X)   [circle]              {$\mathcal{X}$};
\node (mu)  [circle, right=of X]  {$\mu$};
\node (rho) [circle, below=of mu] {$\rho$};
\ifincZ
  \node (Z)   [circle, below=of X]  {$\mathcal{Z}$};
\fi
\node (microscopic)  [left=of X]                          {microscopic};
\node (macroscopic)  [below=of microscopic]               {macroscopic};
\node (particle)     [above=of X, rotate=90, anchor=mid]  {particle};
\node (distribution) [above=of mu, rotate=90, anchor=mid] {distribution};
% arrows
\ifdirect
  \draw [->, out=120,in=-30] (rho.north)     to node [swap] {$\oper{M}{c}{p}$} (X.east);
  \draw [-,  out=30,in=90]   (X.north east)  to ($(X)!.5!(mu)$);
  \draw [->, out=-90,in=-30] ($(X)!.5!(mu)$) to (X.east);
\else
  \draw [->, out=60,in=-60]   (rho.north east)  to node [swap] {$\oper{M}{c}{f}_1$} (mu.south east);
  \draw [-,  out=-120,in=180] (mu.south)        to ($(rho)!.5!(mu)$);
  \draw [->, out=0,in=-60]    ($(rho)!.5!(mu)$) to (mu.south east);
  \draw [->, out=150,in=30]   (mu.north west)   to node [swap] {$\oper{M}{f}{p}_2$} (X.north east);
  \draw [-,  out=-30,in=-90]  (X.east)          to ($(X)!.5!(mu)$);
  \draw [->, out=90,in=30]    ($(X)!.5!(mu)$)   to (X.north east);
  \draw [->, out=-30,in=-150] (X.south east)    to node [swap] {} (mu.south west);
\fi  

\ifincZ
  \draw [->, out=-120,in=120] (X.south west)  to node [swap] {$\oper{R}{p}{n}_1$} (Z.north west);
  \draw [->, out=-30,in=-150] (Z.south east)  to node [swap] {$\oper{R}{n}{c}_2$} (rho.south west);
\else
  \draw [->, out=-60,in=150]  (X.south)       to node [swap] {$\oper{R}{p}{c}$} (rho.west);
\fi
\end{tikzpicture}


==> for arXiv/jump_cdf.tikz.tex <==
\newcommand\drawjumpcdf[1]{
\pgfplotstableread[col sep=comma]{csv/interleaved#1.csv}\meshtable
\pgfplotstableread[col sep=comma]{csv/edges#1.csv}\edgestable
\begin{axis}[
axis lines=left, xmin=-3,xmax=3,ymin=0.0,ymax=0.5,
xlabel={$x$}, ylabel={pdf},
width=7cm, height=5cm, 
name=meshaxis#1
]
\addplot [KULeuvenBlauw, thick,mark=none] table [%
x=x,%
y=f,%
col sep=comma] {\meshtable};
\addplot [KULeuvenLichtblauw, thick,mark=none] table [%
x=x,%
y=g,%
col sep=comma] {\meshtable};
\addplot [KULeuvenRechtsgeleerdheid, thick,mark=none] table [%
x=x,%
y=h,%
col sep=comma] {\meshtable};
\addplot [KULeuvenIngenieurswetenschappen, thick,mark=none] table [%
x=x,%
y=rho,%
col sep=comma] {\meshtable};
\end{axis}%
\begin{axis}[
axis lines=left, xmin=-3,xmax=3,ymin=0.0,ymax=1.0, 
xlabel={}, ylabel={cdf},
width=7cm, height=5cm, 
name=edgesaxis, anchor=south, at={(meshaxis#1.north)}
]
\addplot [KULeuvenBlauw, thick,mark=none] table [%
x=x,%
y=F,%
col sep=comma] {\edgestable};
\addplot [KULeuvenBlauw, thick, only marks, mark color=yellow,mark=-] table [%
x=xF,%
y=H,%
col sep=comma] {\edgestable};
\addplot [KULeuvenLichtblauw, thick,mark=none] table [%
x=x,%
y=G,%
col sep=comma] {\edgestable};
\addplot [KULeuvenLichtblauw, thick, only marks, mark color=black,mark=-] table [%
x=xG,%
y=H,%
col sep=comma] {\edgestable};
\addplot [KULeuvenRechtsgeleerdheid, thick,mark=*] table [%
x=x,%
y=H,%
col sep=comma] {\edgestable};
\addplot [black!20, thick, mark=square*] table [%
x=xH_before,%
y=H,%
col sep=comma] {\edgestable};
\addplot [KULeuvenIngenieurswetenschappen, thick, mark=square*] table [%
x=xH,%
y=H,%
col sep=comma] {\edgestable};
%\csvreader[head to column names]{edges.csv}{}%
%{%
%\pgfmathsetmacro\xHt{\thecsvrow/10-1}%
%\pgfmathsetmacro\Ht{\thecsvrow/5-4}%
%\typeout{\xHt}%
%\node at (\xHt,\Ht) {x};%
%%[circle, fill=KULeuvenLichtblauw, text=white, inner sep=.05cm] 
%}
\end{axis}%
}

%\begin{tikzpicture}
%\node (pic1) {\drawjumpcdf{}};
%\node (pic2) [right=of pic1] {\drawjumpcdf{_adv}};
%\node (pic3) [right=of pic2] {\drawjumpcdf{_degen}};
%\end{tikzpicture}
\resizebox{0.9\textwidth}{!}{%
\begin{tikzpicture}
\drawjumpcdf{}
\end{tikzpicture}
\begin{tikzpicture}
\drawjumpcdf{_adv}
\end{tikzpicture}
\begin{tikzpicture}
\drawjumpcdf{_degen}
\end{tikzpicture}
}


==> for arXiv/macros.tex <==
% New definition of square root:
% it renames \sqrt as \oldsqrt
\let\oldsqrt\sqrt
% it defines the new \sqrt in terms of the old one
\def\sqrt{\mathpalette\DHLhksqrt}
\def\DHLhksqrt#1#2{%
\setbox0=\hbox{$#1\oldsqrt{#2\,}$}\dimen0=\ht0
\advance\dimen0-0.2\ht0
\setbox2=\hbox{\vrule height\ht0 depth -\dimen0}%
{\box0\lower0.4pt\box2}}
%
\newcommand{\DS}{\displaystyle}
\newcommand{\TS}{\textstyle}
\DeclareMathOperator{\spanop}{span}

%
% Fettgedruckte mathematische Symbole (Vektoren, Tensoren)
%

\newcommand{\deltabf}{\boldsymbol{\delta}}
\newcommand{\zetabf}{\boldsymbol{\zeta}}
\newcommand{\taubf}{\boldsymbol{\tau}}
\newcommand{\Phibf}{\boldsymbol{\Phi}}
\newcommand{\omegabf}{\boldsymbol{\omega}}

\newcommand{\nablabf}{\boldsymbol{\nabla}}
\newcommand{\nablabfs}{\boldsymbol{\nabla}_{\!s}}

%
% Kennzahlen
%
\renewcommand{\Re}{\textrm{Re}}
\newcommand{\We}{\textrm{We}}
\newcommand{\Str}{\textrm{Str}}
\newcommand{\Eu}{\textrm{Eu}}
\newcommand{\On}{\textrm{On}}
\newcommand{\La}{\textrm{La}}
\newcommand{\Bo}{\textrm{Bo}}
\newcommand{\Eo}{\textrm{Eo}}
\newcommand{\WeRe}{\text{$\We\Re^{-0.5}$}}
%\newcommand{\WeReI}{\text{$\We_0\Re^{-0.5}_0$}}
\newcommand{\WeReI}{\text{$\We\Re^{-0.5}$}}
\newcommand{\Tu}{\textit{Tu}}
%\newcommand{\Wecorr}{\tilde{\We}}
\newcommand{\Wecorr}{\We^*}

% Differentialoperatoren
%
% ersterOrdnung
\newcommand{\ddt}{\frac{\DS \partial}{\DS \partial t}}
\newcommand{\ddx}{\frac{\DS \partial}{\DS \partial x}}
\newcommand{\ddy}{\frac{\DS \partial}{\DS \partial y}}
\newcommand{\ddz}{\frac{\DS \partial}{\DS \partial z}}
\newcommand{\ddr}{\frac{\DS \partial}{\DS \partial r}}
\newcommand{\ddp}{\frac{\DS \partial}{\DS \partial \theta}}
\newcommand{\ddT}[1]{\frac{\DS \partial #1}{\DS \partial t}}
\newcommand{\ddR}[1]{\frac{\DS \partial #1}{\DS \partial r}}
\newcommand{\ddP}[1]{\frac{\DS \partial #1}{\DS r\partial \theta}}
\newcommand{\ddQ}[1]{\frac{\DS \partial #1}{\DS \partial \theta}}

% hherer Ordnung
\newcommand{\Ddr}{\frac{\DS \partial^2}{\DS \partial r^2}}
\newcommand{\DdT}[1]{\frac{\DS \partial^2 #1}{\DS \partial t^2}}

%
% Integraloperatoren
%

\newcommand{\intV}{\int \limits_{V}}
\newcommand{\intA}{\int \limits_{A}}

\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\var}{{\rm var}}

%
% pstricks
%
%\newpsobject{showgrid}{psgrid}{subgriddiv=1,griddots=10,gridlabels=6pt}

%
% Sonstige
%

\newcommand{\artanh}{\mathop{\mathrm{artanh}}\nolimits} % artanh
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\Tdef}{T_{\text{\it def}}}
\newcommand{\Def}{\text{\it def}}
\newcommand{\xq}{\overline{x}}
\newcommand{\yq}{\overline{y}}
\newcommand{\zq}{\overline{z}}
\newcommand{\Sq}{\overline{S}}
% underbracing with struts 
\newcommand{\bracebox}[3]{\underbrace{\mbox{\rule[-#1mm]{0mm}{#1mm}}#2}_{#3}}

%\newcommand\ointint{\begingroup \displaystyle \unitlength 1pt
% \int\mkern-7.2mu\begin{picture}(0,3)\put(0,3){\oval(10,8)}\end{picture}
% \mkern-7mu\int\endgroup}

% dasdot style fuer PStricks
\makeatletter
\def\psls@dotteddashed{%
[ 0 \psk@dotsep CLW add \psk@dash ] 0 setdash  1 setlinecap  stroke}
\makeatother

\newcommand{\dd}{\,\mathrm{d}}
\newcommand{\DD}{\,\mathrm{D}}
\newcommand{\bs}[1]{\boldsymbol{#1}}

\newcommand{\unit}[1]{\,\mathrm{\left[#1\right]}}

\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pdd}[3]{\frac{\partial^2 #1}{\partial #2 \partial #3}}
\newcommand{\pds}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\fd}[2]{\frac{\dd #1}{\dd #2}}
\newcommand{\fdd}[3]{\frac{\dd^2 #1}{\dd #2 \dd #3}}
\newcommand{\fds}[2]{\frac{\dd^2 #1}{\dd^2 #2}}
\newcommand{\md}[2]{\frac{\DD #1}{\DD #2}}
\newcommand{\mdd}[3]{\frac{\DD^2 #1}{\DD #2 \DD #3}}
\newcommand{\mds}[2]{\frac{\DD^2 #1}{\DD^2 #2}}
\newcommand{\vd}[2]{\frac{\delta #1}{\delta #2}}
\newcommand{\vdd}[3]{\frac{\DD^2 #1}{\delta #2 \delta #3}}
\newcommand{\vds}[2]{\frac{\delta^2 #1}{\delta^2 #2}}

\newcommand{\poibra}[2]{\left\lbrace #1 , #2 \right\rbrace}
\newcommand{\poitrp}[3]{\poibra{\poibra{#1}{#2}}{#3}}
\newcommand{\ensbra}[1]{\left\langle #1 \right\rangle}
\newcommand{\combra}[2]{\left[ #1, #2 \right]}
\newcommand{\inprod}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\expbra}[1]{\mathbb{E} \left[ #1 \right]}
\newcommand{\liealg}[2]{\mathcal{L}\left\lbrace #1 , #2 \right\rbrace}
\newcommand{\commut}[2]{\left[#1 , #2 \right]}
\newcommand{\intseq}[2]{\left\lbrace #1,\ldots,#2 \right\rbrace}
\newcommand{\ensemble}[2]{\left\lbrace #1 \right\rbrace_{#2}}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "text.tex"
%%% End: 

\newcommand{\Oh}[1]{\mathcal{O}(#1)}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\ii}{\mathrm{i}}
\newcommand{\IR}{\mathbb{R}}
\newcommand{\IS}{\mathbb{S}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\diag}{diag}


==> jump_cdf.tikz.tex <==
\newcommand\drawjumpcdf[1]{
\pgfplotstableread[col sep=comma]{csv/interleaved#1.csv}\meshtable
\pgfplotstableread[col sep=comma]{csv/edges#1.csv}\edgestable
\begin{axis}[
axis lines=left, xmin=-3,xmax=3,ymin=0.0,ymax=0.5,
xlabel={$x$}, ylabel={pdf},
width=7cm, height=5cm, 
name=meshaxis#1
]
\addplot [KULeuvenBlauw, thick,mark=none] table [%
x=x,%
y=f,%
col sep=comma] {\meshtable};
\addplot [KULeuvenLichtblauw, thick,mark=none] table [%
x=x,%
y=g,%
col sep=comma] {\meshtable};
\addplot [KULeuvenRechtsgeleerdheid, thick,mark=none] table [%
x=x,%
y=h,%
col sep=comma] {\meshtable};
\addplot [KULeuvenIngenieurswetenschappen, thick,mark=none] table [%
x=x,%
y=rho,%
col sep=comma] {\meshtable};
\end{axis}%
\begin{axis}[
axis lines=left, xmin=-3,xmax=3,ymin=0.0,ymax=1.0, 
xlabel={}, ylabel={cdf},
width=7cm, height=5cm, 
name=edgesaxis, anchor=south, at={(meshaxis#1.north)}
]
\addplot [KULeuvenBlauw, thick,mark=none] table [%
x=x,%
y=F,%
col sep=comma] {\edgestable};
\addplot [KULeuvenBlauw, thick, only marks, mark color=yellow,mark=-] table [%
x=xF,%
y=H,%
col sep=comma] {\edgestable};
\addplot [KULeuvenLichtblauw, thick,mark=none] table [%
x=x,%
y=G,%
col sep=comma] {\edgestable};
\addplot [KULeuvenLichtblauw, thick, only marks, mark color=black,mark=-] table [%
x=xG,%
y=H,%
col sep=comma] {\edgestable};
\addplot [KULeuvenRechtsgeleerdheid, thick,mark=*] table [%
x=x,%
y=H,%
col sep=comma] {\edgestable};
\addplot [black!20, thick, mark=square*] table [%
x=xH_before,%
y=H,%
col sep=comma] {\edgestable};
\addplot [KULeuvenIngenieurswetenschappen, thick, mark=square*] table [%
x=xH,%
y=H,%
col sep=comma] {\edgestable};
%\csvreader[head to column names]{edges.csv}{}%
%{%
%\pgfmathsetmacro\xHt{\thecsvrow/10-1}%
%\pgfmathsetmacro\Ht{\thecsvrow/5-4}%
%\typeout{\xHt}%
%\node at (\xHt,\Ht) {x};%
%%[circle, fill=KULeuvenLichtblauw, text=white, inner sep=.05cm] 
%}
\end{axis}%
}

%\begin{tikzpicture}
%\node (pic1) {\drawjumpcdf{}};
%\node (pic2) [right=of pic1] {\drawjumpcdf{_adv}};
%\node (pic3) [right=of pic2] {\drawjumpcdf{_degen}};
%\end{tikzpicture}
\resizebox{0.9\textwidth}{!}{%
\begin{tikzpicture}
\drawjumpcdf{}
\end{tikzpicture}
\begin{tikzpicture}
\drawjumpcdf{_adv}
\end{tikzpicture}
\begin{tikzpicture}
\drawjumpcdf{_degen}
\end{tikzpicture}
}

